Minimizing Information Leakage of Abrupt Changes in Stochastic Systems

This work investigates the problem of analyzing privacy of abrupt changes for general Markov processes. These processes may be affected by changes, or exogenous signals, that need to remain private. Privacy refers to the disclosure of information of these changes through observations of the underlying Markov chain. In contrast to previous work on privacy, we study the problem for an online sequence of data. We use theoretical tools from optimal detection theory to motivate a definition of online privacy based on the average amount of information per observation of the stochastic system in consideration. Two cases are considered: the full-information case, where the eavesdropper measures all but the signals that indicate a change, and the limited-information case, where the eavesdropper only measures the state of the Markov process. For both cases, we provide ways to derive privacy upper-bounds and compute policies that attain a higher privacy level. It turns out that the problem of computing privacy-aware policies is concave, and we conclude with some examples and numerical simulations for both cases.

==> Figures/old/draft.tex <==
% !TeX encoding = UTF-8
% !TeX root = main.tex
% !TeX spellcheck = en_US

\section{Draft}

We are interested in studying the following Gaussian channel
\[Y_t =  
\begin{cases}
U_t + W_t \quad 0\leq  t< t^\star\\
\theta_0 + W_t \quad t\geq t^\star
\end{cases}\]
where $W_t \sim \mathcal{N}(\mu, \sigma^2)$. We assume that $\theta_0$ is a constant and that $U_t$ is sampled from an unknown stationary distribution $P$. We are interested in finding such distribution, under the constraint that $\mathbb{E}[U_t^2]\leq \lambda^2$.

Observe that the pdf of $Y_t$ for $t\geq t^\star$ is simply  $\mathcal{N}(\theta_0+\mu, \sigma^2)$. Let $Y_1$ be sampled from the distribution of $\theta_0+W_t$, whilst $Y_0$ be sampled from $U_t+W_t$. We are interested in the following optimization problem

\begin{equation}
\begin{aligned}
\min_{P} \quad &\kl(Y_1|Y_0)& \\
\textrm{s.t.} \quad & \mathbb{E}_{P}[U_t^2]\leq \lambda^2
\end{aligned}
\end{equation}
Observe that 
\begin{align*}
\kl(Y_1|Y_0)
&= \int_{\mathbb{R}}f_1(y)\ln(f_1(y)/f_0(y)) dy\\
&= -H(Y_1) -\int_{\mathbb{R}}f_1(y)\ln(f_0(y)) dy
\end{align*}
Suppose that $U_t$ is a constant term. It means that $f_0(y) = \frac{1}{\sqrt{2\pi\sigma^2}} e^{-(y-u-\mu)^2/2\sigma^2}$. It follows that

==> Figures/old/full.tex <==
% !TeX encoding = UTF-8
% !TeX root = main.tex
% !TeX spellcheck = en_US

\subsection{Full-information case} \label{sec:full_information}
\textbf{Definitions and introduction. }
In the full-information case the eavesdropper is able to measure both the state and action $(x_t,a_t)$ at time $t$, from which follows that minimizing leakage of information is potentially much harder for the agent. It turns out that the agent is able to affect the quantity $I$ only for some MDPs, whilst for others, such as linear dynamical systems with additive changes, privacy depends solely on the properties of the change, and the stochastic properties of the MDP.

 Without loss of generality consider the case $M_0\to M_1$. For a sequence of observations  $\{X_1,A_1,X_2,\dots, X_t\}$ (measured by the eavesdropper) we can define the following log-likelihood ratio
\begin{equation}
	Z_{i} = \ln \frac{P_1(X_i|X_{i-1}, A_{i-1})}{P_0(X_i|X_{i-1}, A_{i-1})},\quad i\in \{2,\dots, t\}.
\end{equation}
Due to ergodicity  it follows that $n^{-1}\sum_{t=\nu}^{\nu+n} Z_t$ converges to $I_1(\pi_1)$   under $\mathbb{P}_\nu$, where $\mathbb{P}_\nu$ indicates the the probability measure induced by $\pi_1$ in $M_1$, and the quantity $I_1(\pi_1)$ is
\begin{equation}\label{eq:I_full_information}
	I_{1}(\pi_1) = \int_{X\times A} \mathbb{E}_{P_1}[Z_2|X_{1}=x, A_1=a]  \textrm{d}\pi_1(a|x)\textrm{d}\mu_1^{\pi_1}(x).
\end{equation} 
Similarly, for the case $M_1\to M_0$ one can define $I_{0}(\pi_0)$.

An important observation, that we will be using in the following, is that $I_1$ in the full-information case is affected only by $\pi_1$, and not by $\pi_0$ (also the converse holds true). This is a consequence of the assumption  that the adversary is able to observe the sequence of actions taken by the agent.


Based on these quantities, one can define an indicator of hardness, that takes into account both cases $M_0\to M_1$ and $M_1\to M_0$, and that can be thought of being the symmetrised  KL-divergence between the two models.
\begin{definition}
 Let $M=\{M_0, M_1\}$ and $\pi=\{\pi_0,\pi_1\}$. We indicate the overall privacy level for $(M,\pi)$ in the full-information case by
\begin{equation}
\mathcal{I}_F(M,\pi) = I_{1}(\pi_1) +I_{0}(\pi_0).
\end{equation}
\end{definition}

In other words, the lower $\mathcal{I}_F(M,\pi)$, the more difficult is the detection problem for both the cases $M_0\to M_1$ and $M_1\to M_0$. Because of the properties of the KL-divergence, one can immediately observe that $\mathcal{I}_F(M,\pi)$ is non-negative, and that a sufficient condition for  $\mathcal{I}_F(M,\pi)$ being $0$ is that KL divergence of $\xi_1^\pi$ and $\xi_0^\pi$ is $0$. Furthermore, $\mathcal{I}_F(M,\pi)$ is convex in the state-action distributions $(\xi_1,\xi_2)$, where $\xi_i(x,a) = \pi_i(a|x)\mu_i^{\pi_i}(x)$. The fact that $I_i$ depends solely on $\pi_i$ allows us to find the maximum level of privacy by optimizing separately in $\pi_1$ and $\pi_0$, as shown in the following lemma.

\begin{lemma}\label{lemma:lower_bound_privay}
For simplicity, let $X,A$ be finite sets. Given $(M,\pi)$ the maximum level of attainable privacy in the full-information case is
\begin{equation}
\mathcal{I}_F(M) \coloneqq \underbrace{\inf_{\pi_1} I_1(\pi_1)}_{i_1}+ \underbrace{\inf_{\pi_0} I_0(\pi_0)}_{i_0}
\end{equation}
where $i_1$ (similarly $i_0$) is the solution of the following convex program
\begin{equation}\label{eq:min_c1_full_information}
\begin{aligned}
\min_{\xi\in \Delta(X\times A)} \quad & \mathbb{E}_{(x,a) \sim \xi}\left[I\left(P_1(\cdot|x,a), P_0(\cdot|x,a)\right)\right]\\
\textrm{s.t.} \quad & \sum_{a} \xi_{*,a}^\top P_1(a) =\sum_{a} \xi_{*,a}^\top,\\
\end{aligned}
\end{equation}
	with  $P_1(a)$ being a $|X|\times |X|$ matrix containing the transition probabilities for a specific action $a$ in MDP $M_1$.
\end{lemma}
\begin{proof}
The maximum level of privacy is attained when $\mathcal{I}_F(M,\pi)$ is minimum, therefore for $\inf_\pi \mathcal{I}_F(M,\pi) =\inf_{\pi_1,\pi_0} \left(I_1(\pi_1) + I_0(\pi_0)\right)$. Since  $I_1(\pi_1)$ is positive, and does not depend on $\pi_0$ (similar arguments for $I_0$), we  have $\inf_{\pi_1,\pi_0} \left(I_1(\pi_1) + I_0(\pi_0)\right)= \inf_{\pi_1} I_1(\pi_1)+\inf_{\pi_0} I_0(\pi_0)$.
Now, without loss of generality, consider just $i_1$. Observe that $I_1(\pi_1)$ in the discrete case can be rewritten as
\begin{align*}
I_1(\pi_1) &= \sum_{x,a} \mu_1^{\pi_1}(x) \pi_1(a|x) \mathbb{E}_{X_2\sim P_1}[Z_2|X_{1}=x, A_1=a],\\
&=\sum_{x,a} \mu_1^{\pi_1}(x) \pi_1(a|x)\sum_{y} P_1(y|x,a) \ln \frac{P_1(y|x,a)}{P_0(y|x,a)} \\
&=\sum_{x,a} \xi_1(x,a)\sum_{y} P_1(y|x,a) \ln \frac{P_1(y|x,a)}{P_0(y|x,a)} 
\end{align*}
where  $\xi_1(x,a)\coloneqq\pi_1(a|x)\mu_1^{\pi_1}(x)$. To conclude the proof, notice that $\xi_1$ must satisfy the constraint that $\mu_1^{\pi_1}$ is a stationary distribution. Therefore minimizing $I_1(\pi_1)$ is equivalent to minimizing the last equation over $\xi_1\in \Delta(X\times A)$, subject to $\sum_{a} \xi_{*,a}^\top P_1(a) =\sum_{a} \xi_{*,a}^\top$.
\end{proof}
\textbf{Privacy in exponential systems. }Unfortunately $\underline{\mathcal{I}}_F(M)$ depends on the type of MDP being controlled, and the constants $i_1,i_0$ cannot be computed without further assumptions on the model. In case of exponential models where the change is not state/action dependent we have the following corollary.
\begin{corollary}\label{corollary:constant_privacy}
Consider  lemma \ref{lemma:lower_bound_privay}. Suppose $P_1(\cdot|x,a)$ and $P_0(\cdot |x,a)$ to be exponential distributions parametrized by two parameters $\theta_{1},\theta_{0}\in \mathbb{R}^k$, such that $P_{i}(y|x,a) = P_{\theta_i}(y|x,a)$ and
\[P_{\theta_i}(y|x,a)= h(y)\exp\left(\langle \theta_i, T_{x,a}(y)\rangle + A(\theta_{i}) \right)\]
where $T_{x,a}(y)$ is a sufficient statistics, $\theta_i$ is a natural parameter that does not depend on $(x,a)$, $A(\theta_i)$ is the log partition function and $h(y)$ is a non-negative function. It follows that $i_1 = (A(\theta_{1}) - A(\theta_{0})) + \langle\eta(\theta_{1}) - \eta(\theta_{0}), \nabla A(\theta_1)\rangle =D_A(\theta_1,\theta_0)$  (similarly $i_0$), where $D_A(z,w)$ denotes the Bregman Divergence associated with $A$ for points $z,w\in \mathbb{R}^k$. Therefore the maximum level of attainable privacy is 
\begin{equation}
\underline{\mathcal{I}}_F(M) =  D_A(\theta_1,\theta_0)+D_A(\theta_0,\theta_1).
\end{equation}
\end{corollary}
\begin{proof}
Consider the constant $i_1$. The the log-likelihood ratio is simply
\begin{align*}
\ln \frac{P_1(y |x,a)}{P_0(y |x,a)} = \langle \theta_1-\theta_0, T_{x,a}(y)\rangle + A(\theta_{1}) - A(\theta_{0}).
\end{align*}
Since $\mathbb{E}_{y\sim P_i(\cdot|x,a)}[T_{x,a}(y)] = \nabla_\theta A(\theta_i)$, due to linearity it follows that
\begin{align*}
\mathbb{E}_{y\sim P_1(\cdot|x,a)}\left[\ln \frac{P_1(y |x,a)}{P_0(y |x,a)}\right] &= \langle \theta_1-\theta_0, \nabla_{\theta} A(\theta_1)\rangle \\&\quad+ A(\theta_{1}) - A(\theta_{0}).
\end{align*}
The last expression does not depend on $(x,a)$, therefore we must conclude that 
\begin{align*}
i_1 &=  \langle \theta_1-\theta_0, \nabla_{\theta} A(\theta_1)\rangle + A(\theta_{1}) - A(\theta_{0}) =D_A(\theta_1,\theta_0)\\
i_0 &=  \langle \theta_0-\theta_1, \nabla_{\theta} A(\theta_0)\rangle + A(\theta_{0}) - A(\theta_{1})=D_A(\theta_0,\theta_1)
\end{align*}
and thus $i_1+i_0 = \langle \theta_1-\theta_0, \nabla_{\theta} (A(\theta_1) -  A(\theta_0))\rangle$.
\end{proof}
The previous corollary sheds a light on the interesting case where the change is not affected by the current state/action pairs. For this particular case privacy depends solely on the difference of the natural parameters, scaled by the sensitivity of the log-partition function to change in the natural parameters. This result holds, for example, for linear dynamical systems affected by an additive change, whilst it does not hold for multiplicative changes.

\textbf{Privacy-utility trade-off.} Now that we performed an initial analysis of the problem, we are ready to tackle the utility-privacy trade-off problem. Computing a policy that only minimizes information leakage is per-se interesting, but in most cases useless since the agent is also interested in maximizing the collected reward. For sake of notation, let $T_1(x,a,y) = P_1(y|x,a) \ln \frac{P_1(y|x,a)}{P_0(y|x,a)}$ and $T_0(x,a,y)=P_0(y|x,a) \ln \frac{P_0(y|x,a)}{P_1(y|x,a)}$. The problem of maximizing reward collection whilst minimizing information leakage (in the full-information case) for MDP $M_i$ can be cast to a convex optimization problem, with a constraint on the privacy level as follows 
\begin{equation}
\max_{\pi_i: I_i(\pi_i)\leq \alpha_i }   \lim_{N\to \infty} \mathbb{E}_{M_i}^{\pi_i}\left[\frac{1}{N}\sum_{t=1}^N r_i(s_t,a_t)\right],
\end{equation}
for some $\alpha_i \in \mathbb{R}^+$, $i=1,2$. Using lemma \ref{lemma:lower_bound_privay}, observe that the policy optimization problem is  equivalent to the following  \cite{puterman2014markov}
\begin{equation}
\begin{aligned}
\max_{\xi\in \Delta(X\times A)} \quad & \sum_{x,a} \xi_{x,a}r_i(x,a)\\
\textrm{s.t.} \quad & \sum_{a} \xi_{*,a}^\top P_i(a) =\sum_{a} \xi_{*,a}^\top,\\
  & \sum_{x,a} \xi_{x,a}\sum_{y} T_i(x,a,y) \leq \alpha_i
\end{aligned}
\end{equation}
where the policy $\pi_i$ can be obtained by $\pi_i(a|x) = \dfrac{\xi_{x,a}}{\|\xi_{x,*}\|_1}$.
It follows that for a suitable Lagrange multiplier $\lambda \geq 0$ we can move the privacy constraint into the main objective, so that the problem is equivalent to solving an MDP $(X,A,P_i, r_i^\lambda)$ where the reward is now given by
\[r_i^\lambda(x,a) = r_i(x,a)-\lambda\sum_{y}T_i(x,a,y)\]
and the policy can be computed by solving the following convex program
\begin{equation}
\max_{\xi\in \Delta(X\times A)}  \sum_{x,a} \xi_{x,a}r_i^\lambda(x,a) \quad \textrm{s.t.}\quad \sum_{a} \xi_{*,a}^\top P_i(a) =\sum_{a} \xi_{*,a}^\top,
\end{equation}

\subsubsection{Example: case of additive changes in linear dynamical systems}
Here we investigate an additive change in an $n$-dimensional process $(x_t)_t$ described by the following state-space model
\[x_{t+1} = Ax_t + Ba_t + F\theta \indi_{\{t\geq \nu\}} + w_t\]
where $(a_t)_t$ is the control signal, and $(w_t)_t$ is a white noise sequence with $0$ mean and covariance $Q$. The parameter $\theta \in \mathbb{N}$ models the exogenous input, that is unobservable for the eavesdropper. One can immediately observe that the model is a particular case of corollary \ref{corollary:constant_privacy}, therefore the level of privacy is constant and depends solely on $F,\theta$ and $Q$. To see this, notice that the conditional densities for the two cases are:
\begin{align*}
P_1: x'|(x,a) &\sim \mathcal{N}(Ax+Ba+F\theta, Q)\\
P_0 :x'|(x,a) &\sim \mathcal{N}(Ax+Ba, Q)
\end{align*}
from which follows that 
\begin{align*}
\int_{\mathbb{R}^n}P_1(x'|x,a)\ln \frac{P_1(x'|x,a)}{P_0(x'|x,a)} \textrm{d}x'&=\theta^\top F^\top Q^{-1} F\theta
\end{align*}
therefore the privacy level depends solely on the signal-to-noise ratio (SNR) $\theta^\top F^\top Q^{-1} F\theta$, that is maximum if $F\theta \in \ker(Q^{-1})$.
